Partial Symmetry Detection for 3D Geometry using Contrastive Learning with Geodesic Point Cloud Patches

Detecting partial extrinsic symmetry in 3D geometry is a fundamental yet persistent challenge in computer vision and graphics, critical for tasks ranging from shape completion to procedural generation. Classical transformation-space voting methods rely on pairwise matching, scaling as O(n^2) and struggling to resolve coherent multi-instance groups. Recent learning approaches advance global symmetry detection but restrict the solution space to reflection planes, failing to capture rotational or translational repetitions such as the legs of a chair or the steps of a staircase. We propose SymCL, a self-supervised contrastive learning framework that detects partial symmetries across rotation, translation, and reflection (with scale-invariant features) and requires no ground truth annotations. By mapping local geodesic patches to a latent space invariant to the Euclidean group, we reformulate symmetry detection as a density-based clustering problem, enabling the simultaneous discovery of multi-instance symmetric relationships in a single forward pass. We evaluate quantitatively on SymPartNet, a new benchmark annotating all PartNet categories with partial symmetry relations, and demonstrate class-agnostic generalization qualitatively on everyday objects outside the training distribution.

==> tab/ablation_psb.tex <==
\begin{tabular}{lcccc}
    \toprule
    \multicolumn{5}{c}{\textbf{SymPartNet (Full)}}                      \\
                     & ICP (↓) & IoU (↑) & COV (↑) & \#M. \\
    \midrule
    SymCL (base)     & 0.0024  & \textbf{0.3747}  & 0.8217  & 966  \\
    - offset center  & \textbf{0.0022}  & 0.3683  & 0.7344  & 863  \\
    - scaling        & 0.0025  & 0.3412  & 0.8087  & 982  \\
    - reflections    & 0.0024  & 0.3600  & 0.8207  & 976  \\
    - multiple sizes & 0.0024  & 0.3559  & \textbf{0.8390}   & 983  \\
    \midrule
    Euclidean        & 0.0027  & 0.3446  & 0.8223  & 983  \\
    \bottomrule
\end{tabular}

==> tab/ablation_pspsb.tex <==
\begin{tabular}{lcccc}
    \toprule
    \multicolumn{5}{c}{\textbf{SymPartNet (Parts)}}                    \\
                     & ICP (↓) & IoU (↑) & COV (↑) & \#M. \\
    \midrule
    SymCL (base)     & 0.0028  & 0.7663  & 0.7727  & 969  \\
    - offset center  & 0.0063  & 0.6846  & 0.6317  & 877  \\
    - scaling        & \textbf{0.0019}  & \textbf{0.7789}  & \textbf{0.8031}  & 976  \\
    - reflections    & 0.0023  & 0.7649  & 0.7737  & 976  \\
    - multiple sizes & 0.0024  & 0.7582  & 0.7489  & 928  \\
    \midrule
    Euclidean        & 0.0025  & 0.7631  & 0.7722  & 965  \\
    \bottomrule
\end{tabular}

==> tab/benchmark_chair.tex <==
\begin{tabular}{cccccc}
  \toprule
            & \multicolumn{2}{c}{\textbf{PSPSB}} & \multicolumn{2}{c}{\textbf{PSB}} \\
            & SymCL  & SymML  & SymCL  & SymML   \\
  \midrule
  ICP (↓)   & 0.0028 & 0.0018 & 0.0024 & 0.0023 \\
  IoU (↑)   & 0.7663 & 0.7783 & 0.3747 & 0.3753 \\
  COV (↑)   & 0.7727 & 0.7333 & 0.8217 & 0.8293 \\
  \#Models  & 969    & 894    & 966    & 965    \\
  \bottomrule
\end{tabular}

